Exponential Resummation of QCD at finite chemical potential

A comprehensive study of the QCD phase diagram is one of the challenging and open problems in high energy physics. Having significant astrophysical implications, this is also important in constructing the chronological evolution of the universe. With this aim, this thesis describes the behaviour of thermodynamic observables like pressure and number density with changing chemical potential $\mu$, through the method of an unbiased exponential resummation of lower order Taylor series of these observables at a finite $\mu$. We address the problem of biased estimates, which manifest uncontrollably in exponential resummation and which become severe in the domain of large values, higher orders of $\mu$ and also in observables which are higher $\mu$ derivatives of the thermodynamic potential. We show that our new formalism of unbiased exponential resummation can eliminate these biased estimates exactly upto a given order of $\mu$, and can capture important contributions of higher order Taylor series for all our working temperatures starting from hadronic phase to the plasma phase, including the crossover region. We also demonstrate that this new formalism is highly efficient in saving appreciable computational time and storage space for computations.

==> Back/listofpublications.tex <==
\chapter*{List of Publications} \label{publications}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\rule{\linewidth}{2pt}
%\vspace{5mm}
\textbf{{\large Referred journals:}}
\begin{enumerate}[label=\textbf{[\arabic*]}]
\item A and B, ``Methods to improve Speech Recognition'',
\emph{Artificial Intelligence Review} (2022), Springer.
\url{https://doi.org/10.15}.

\end{enumerate}
\noindent\rule{\linewidth}{0.2pt}
%\vspace{5mm}
\textbf{{\large International conferences:}}
\begin{enumerate}[label=\textbf{[\arabic*]}]
\item A and B, ``Methods to improve Speech Recognition'',
\emph{Artificial Intelligence Review} (2022), Springer.
\url{https://doi.org/10.15}.

\end{enumerate}
\noindent\rule{\linewidth}{0.2pt}
%\vspace{5mm}
\textbf{{\large Papers communicated in referred journals:}}
\begin{enumerate}[label=\textbf{[\arabic*]}]
\item A and B, ``Methods to improve Speech Recognition'',
\emph{Artificial Intelligence Review} (2022), Springer.
\url{https://doi.org/10.15}.
\end{enumerate}

==> Front/LOA.tex <==
\clearpage
\printglossary[type=\acronymtype,title=List of Acronyms,toctitle=List of Acronyms]

QCD Quantum Chromodynamics

EoS Equation of state










==> Front/LOS.tex <==
\clearpage
\printglossary[title=List of Symbols,toctitle=List of Symbols]


==> Front/certificate.tex <==
% do not use titlepage environment, because it does not increase page counter.
%\thispagestyle{}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{center}
{\bf\large CERTIFICATE }\\
\par\vspace{5mm}
\end{center}
\noindent It is certified that work contained in the thesis titled
``\textbf\thetitle{}'' by ``\thescholar'' has been
carried out under my supervision and that this work has not been submitted
elsewhere for a degree.
\vspace{20mm}
% \begin{flushleft}

% \textbf{(Signature of Research Supervisor)}
% \end{flushleft}
\begin{flushleft}
\textbf{\thesupervisor\\
Professor,\\Dept. of Electronics and Communication Engineering\\ Govt.
Engineering College, Thrissur}
\vspace{1cm}

\textbf{\thecosupervisor\\
Professor,\\Dept. of Electronics and Communication Engineering\\ Govt.
Engineering College, Thiruvananthapuram}

\end{flushleft}
\vspace{5mm}

% \begin{flushleft}

% Place: \\
% Date:
% \end{flushleft}
%\vspace*{\fill}
%\vspace{15mm}
% \begin{flushleft}
% \textbf{(Signature of Research Co-Supervisor)}
% \end{flushleft}
%\begin{flushleft}
% \textbf{Dr. Santhoshkumar S.\\
% Professor and Head,\\Dept. of Electronics and Communication
%Engineering\\ Govt. Engineering College, Idukki}
% \end{flushleft}

\begin{flushleft}
\vspace{25mm}
\begin{tabular}{@{}p{1cm}p{5cm}@{}}
Date: & \hrulefill\\
& \\
Place: & \hrulefill\\
\end{tabular}
\end{flushleft}

==> Preamble/packages.tex <==
\NeedsTeXFormat{LaTeX2e}
\usepackage{authblk,lineno,color,lscape,url}
\usepackage[hidelinks]{hyperref}
\usepackage[dvipsnames]{xcolor}
\usepackage[labelfont=bf]{caption}
\usepackage{emptypage}
\usepackage{array,float,multirow,graphicx,setspace,cite,url,titlesec,tocloft}
\usepackage{amsmath,amsfonts,mathtools,notoccite,cleveref}
\usepackage{chngcntr,rotating,pdflscape,enumitem,algpseudocode,algorithm,subcaption}
\usepackage{relsize}
\usepackage{ragged2e}
\usepackage{threeparttable}
\usepackage{tabulary}
\usepackage{booktabs}
\usepackage{amsbsy}
\usepackage{breqn}
\usepackage{amssymb}
\usepackage{calc}
\usepackage{colortbl}


\definecolor{mygreen}{rgb}{0.7, 1, 0.}
\definecolor{myred}{rgb}{1.0, 0.8, 0.7}
\definecolor{myyellow}{rgb}{1.0, 1.0, 1.0}
\definecolor{myblue}{rgb}{0.3, 0.7, 1.0}
%\usepackage{mathrsfs}
% \usepackage{nccmath}
\usepackage[skip=5pt plus1pt, indent=20pt]{parskip}
\usepackage{setspace}
\usepackage{exscale}
\usepackage{array}
\usepackage{relsize}
\usepackage{feynmp-auto}
\usepackage{tikz}
\usepackage{float}
\usepackage[numbers,square,compress]{natbib}
\usepackage{cite}
\usepackage{fancyhdr}
\usepackage{hyperref}
\usetikzlibrary{shapes,arrows,
                positioning,
                }

\usepackage[nottoc]{tocbibind}

\usepackage{pst-node}
\def\data#1{%
     \pspicture(-0.45,-0.5)(0.45,0.5)
     \psline(-0.45,0.5)(-0.45,-0.5)\psellipticarc(0,-0.5)(0.45,0.1){180}{0}\psline(0.45,-0.5)(0.45,0.5)
     \psellipse(0,0.5)(0.45,0.1)\rput(0,0){#1}
     \endpspicture}


\usepackage [autostyle, english = american]{csquotes}
\MakeOuterQuote{"}

 \hypersetup{
    final=true,
    plainpages=false,
    pdfstartview=FitV,
    pdftoolbar=true,
    pdfmenubar=true,
    bookmarksopen=true,
    bookmarksnumbered=true,
    breaklinks=true,
    linktocpage,
    colorlinks=true,
    linkcolor=red,
    urlcolor=red,
    citecolor=red,
    anchorcolor=red
  }

